On the Importance of Contrastive Loss in Multimodal Learning

Recently, contrastive learning approaches (e.g., CLIP (Radford et al., 2021)) have received huge success in multimodal learning, where the model tries to minimize the distance between the representations of different views (e.g., image and its caption) of the same data point while keeping the representations of different data points away from each other. However, from a theoretical perspective, it is unclear how contrastive learning can learn the representations from different views efficiently, especially when the data is not isotropic. In this work, we analyze the training dynamics of a simple multimodal contrastive learning model and show that contrastive pairs are important for the model to efficiently balance the learned representations. In particular, we show that the positive pairs will drive the model to align the representations at the cost of increasing the condition number, while the negative pairs will reduce the condition number, keeping the learned representations balanced.

==> related-works.tex <==
\section{Introduction}



One of the exceptional abilities of humans is to associate data from different modalities (such as texts and images) together. When we hear the words ``white dog'', we can immediately align it with the image of a white dog. 

Recently, multi-modality learning method: Training the model to be able to align the data from different modules have becoming an increasingly popular research direction, especially in deep learning (cite some practical works). Among them, the recent work CLIP~\cite{} shows remarkable quality results to align the features of text and images. The \emph{contrastive learning} based method CLIP empirically outperforms many existing non-contrastive approaches (cite existing approaches). The major difference between contrastive approach and other approaches is that contrastive loss not only requires the learned representation from the same pair of data (i.e. positive pairs) to be positively aligned, but it also requires the data from different pairs (i.e. negative pairs) to be as negatively aligned as possible. In the paper, the authors also identify contrastive loss as the most critical part to the success of CLIP.


Empirical, CLIP has shown superior performance in multi-modality learning to align features from the two modules. For example, the trained model can align the representation of words ``black cat'' with the representation of an image with a black cat, while aligning the words ``yellow cat'' with an image with a yellow cat. However, from a theoretical perspective, the most fundamental  questions are still largely open: In particular, how does the new technique based on negative pairs help in multi-modality learning? How can the \textbf{non-convex} contrastive loss be minimized efficiently to learn features from both modules?


Unlike the prior theoretical works on contrastive learning which mostly focus on extracting features from one module (cite), the main technical challenge of analyzing contrastive learning in multi-modality setting is how the model can be trained to align the feature representations $\phi_1, \phi_2$ from module one and two respectively. Due  to the existence of negative pairs that emphasize on negative correlations of $\phi_1$ and $\phi_2$, it is unclear that the model is still incentive to align them.


In this paper we make preliminary theoretical steps towards answering the fundamental theoretical questions of contrastive loss in multi-modality learning. We adopt the theoretical framework from the seminal work (cite), which assumes that the data is coming from $X = Az + \xi$. Here, $z$ is considered as the hidden signal, $A$ is a (linear) transformation from the signal to the observation, and $\xi$ is the noise. In our case, we assume that the data from the two modalities are of form $X_1 = Az + \xi$ and $X_2 = Bz + \xi'$ respectively. The positive pair of the data shares the same signal $z$, and differ from the noise $\xi$ and the transformations $A, B$. The goal is to learn features $\phi_1, \phi_2$ that aligns data from the two modules. 


Under this setting, we make the following contributions:

\begin{enumerate}
    \item We consider the challenging (but more practical) setting where the features in $A$ and $B$ are inhomogenous, meaning that the condition number of $A$ and $B$ can be $\omega(1)$. Prior works (cite) only considers when $A$ and $B$ are exactly column orthogonal matrices with condition number $1$ even in the simpler setting of single modality ($A = B$).
    \item We consider the feature learners $\phi_1, \phi_2$ with normalization, meaning that $\phi_1, \phi_2$ are always normalized to have (expected) norm one during training. Output normalization plays a critical rule in the practical success of contrastive learning, but it is rarely considered in theory due to  the additional complexity of the division. 
    \item We analyze the learning process of stochastic gradient descent from random initialization. We prove that contrastive learning converges efficiently to a nearly optimal solution, which indeed aligns the feature representation $\phi_1$ and $\phi_2$.
    
    \item We also demostrate the importance of negative pairs by comparing with training only over the positive pairs. We prove that although the latter can also learn to align $\phi_1$ and $\phi_2$, the features learned by contrastive learning with negative pairs is much more \emph{uniform}. Meaning that $\phi_1, \phi_2$ can recover all the singular vectors of $A$ and $B$. On the other hand, without negative pairs the learned representation is close to a rank one solution, meaning that $\phi_1, \phi_2$ will only focus on the top singular direction of $A$ and $B$. 
    
    \item We perform empirical evaluations in our setting to further support our theory.
\end{enumerate}



\section{Related Works}

\paragraph{Multimodal learning}

You can check this paper 
``What Makes Multi-modal Learning
Better than Single (Provably)'' and the paper that cites this paper. These are the theoretical works in multi-modal learning.  You want to demostrate that they DO NOT consider contrastive learning, but more focus on the traditional method that only emphasize on the positive pairs. 

\paragraph{Contrastive/Non-contrastive learning theory}

We want to demostrate: (1). All of the contrastive learning works only focus on single modality. There, they use just one learner $\phi$, which has no ``feature alignment'' issue. The ``feature alignment'' is the most important focus of our work. 

(2). They either don't consider gradient descent, or they only consider when the features are uniform.

(3). They don't consider output normalization except one recent work by Zixin.




Starting from \cite{arora_theoretical_2019}, many recent works have provided various explanations on why 
the representations learned with contrastive learning are useful in downstream tasks (\cite{chuang_debiased_2020,%
tosh_contrastive_2021,nozawa_understanding_2021,wang_chaos_2022,haochen_provable_2021,lee_predicting_2021}). 
These works mostly focus on the generalization aspect of the problem, and do not provide guarantees on the 
training. Another related line of research is about non-contrastive learning, where the necessity of negative 
examples is questioned. In this line of research, the optimization problem does get considered as
non-contrastive losses have trivial collapsed solutions. \cite{tian_understanding_2021} show that, 
under certain conditions, non-contrastive learning methods can learn non-collapsed solutions. 
\cite{jing_understanding_2022} show that, even with negative examples, contrastive learning can still suffer 
from another type of collapse, where the learned representation only expand a low-dimensional subspace of 
the embedding space. In \cite{pokle_contrasting_2022}, the authors show that non-contrastive losses have 
many non-collapsed bad minima that the training algorithm does not avoid. Another related work that takes 
optimization into consideration is \cite{wen_toward_2021}, in which the authors analyze the training dynamics 
of contrastive learning and show that, with random augmentation, neural networks can learn features that are 
suppressed by noises when no augmentations are used. We compare our result with the most relevant works 
in the next paragraph. 


\paragraph{Comparsion with \cite{jing_understanding_2022,tian_understanding_2021,wen_toward_2021}}
The dimensional collapse problem reported in \cite{jing_understanding_2022} is not a real issue in our 
setting, since, in our case, the best the model can do is to recover the latent vector $\z$, up to some 
rotation. As a result, it is natural for the learned representations to span only a low-dimensional subspace 
of the embedding space $\R^m$. Here, the point of choosing $m \gg d$ is to make the optimization dynamics more 
regular, which is a common strategy in the study of over-parameterized neural networks. The main difference 
between our work and the analysis in \cite{tian_understanding_2021} and \cite{wen_toward_2021} is we do not 
assume the inputs are isotropic. In our setting, the condition number can be as large as $\Theta(\log d)$. 
When the condition number is $1$, one can imagine that, thanks to the symmetry, all directions will be learned 
simultaneously. Therefore, we do not need negative examples to prevent collapse (\cite{tian_understanding_2021})
or the negative examples do not play an important role in analysis (\cite{wen_toward_2021}). On the other hand,
when the condition number is larger than $1$, we do need to use the negative examples to shrink the condition 
number, which corresponds to the second stage of our analysis. 







==> setting.tex <==
\section{Setting}
\TODO{Move the details to appendix.}
Let $r < d$ be two large positive integers. Suppose that the latent vector $\z \in \R^r$ follows 
the uniform distribution over $\{ \pm 1 / \sqrt{d} \}^r$. Let $\A, \B \in \R^{d \times r}$ be two 
encoding matrices with $\A\trans\A = \B\trans\B = \diag(\bsigma^2)$. Let $\A_{\bxi}, \B_{\bxi}
\in \R^{d \times (d - r)}$ be two matrices whose columns are orthogonal to the columns of 
$\A$ and $\B$, respectively. We also assume that $\Axi\trans\Axi = \Bxi\trans\Bxi = \sigma_\xi^2 
\Id_{d-r}$ for some $\sigma_\xi > 0$. These two matrices are used to generate the noises. 

We assume the input samples are generated as follows. First a latent vector $\z \in \R^r$
is sampled. Then we sample $\bxi_{\A}\in \R^{d-r}$ from $\mrm{Unif}\{ \pm 1 / \sqrt{d} \}^{d - r}$,
and concatenate them to form the noisy latent vector $(\z, \bxi_{\A})$. Then we apply the 
concatenated matrix $(\A, \A_{\bxi})$ to it to obtain an input vector $\xA(\z)$. Similarly, 
we can obtain input vectors $\xB(\z)$ with $\B$ and $\B_{\bxi}$. We say that a pair of $\xA$ and 
$\xB$ is a positive pair if they share the same latent vector, and a negative pair if they do not.
In most case, we will use $(\xA^+, \xB^+) = (\xA(\z^+), \xB(\z^+))$ and 
$(\xA^+, \xB^-) = (\xA(\z^+), \xB(\z^-))$ to denote a positive and negative pair, respectively.

The model we consider is 
\[
  \fA(\xA) 
  = \frac{\WA\trans\xA}{\sqrt{\E\norm{\WA\trans\xA}^2}}, \qquad
  \fB(\xB) 
  = \frac{\WB\trans\xB}{\sqrt{\E\norm{\WB\trans\xB}^2}},
\]
where $\WA, \WB \in \R^{d \times m}$ are trainable parameters. Note that 
\begin{align*}
  \E \norm{\WA\trans\xA}^2
  &= \inprod{\WA\WA\trans}{\E\xA\xA\trans} \\
  &= \inprod{\WA\WA\trans}{
      \E\braces{ (\A\z + \A_{\bxi} \bxi_\A)(\A\z + \A_{\bxi} \bxi_\A)\trans }
    } \\
  &= \inprod{\WA\WA\trans}{
      \A \E\braces{\z\z\trans} \A\trans 
      + \underbrace{
          \A \E\braces{\z \bxi_\A\trans} \A_{\bxi}\trans
          + \A_{\bxi} \E\braces{\bxi_\A \z\trans}\A\trans
        }_{=\;0}
      + \A_{\bxi} \E\braces{\bxi_\A \bxi_\A\trans} \A_{\bxi}\trans
    } \\
  &= \frac{1}{d} 
    \left(
      \inprod{\WA\WA\trans}{\A \A\trans}
      + \inprod{\WA\WA\trans}{\A_{\bxi}\A_{\bxi}\trans }
    \right) \\
  &= \frac{\norm{\WA\trans\A}_F^2 + \norm{\WA\trans\A_{\bxi}}^2}{d}.
\end{align*}
The same is also true for $\B$. For notational simplicity, we write $\KA = \WA\trans\A$, 
$\KB = \WB\trans\B$, $\KAxi = \WA\trans\A_{\bxi}$, and $\KBxi = \WB\trans\B_{\bxi}$. For 
notational simplicity, define $N_\A^2 = (\norm{\KA}_F^2 + \norm{\KAxi}_F^2) / d$ and
$N_\B^2 = (\norm{\KB}_F^2 + \norm{\KBxi}_F^2) / d$. Our model is equivalent to 
\[
  \fA(\xA) 
  = \frac{\WA\trans\xA}{ N_\A }, \qquad
  \fB(\xB) 
  = \frac{\WB\trans\xB}{ N_\B }.
\]
We train the model with GF over the population contrastive loss $\Loss$, which is defined as 
follows. First, we define 
\begin{align*}
  S_\A(\xA^+, \xB^+)
  &= \frac{ \exp(\tau_t^2 \fA^+ \cdot \fB^+ ) }
    {\exp(\tau_t^2 \fA^+ \cdot \fB^+ ) + K \E_{\xB^-} \exp(\tau_t^2 \fA^+ \cdot \fB^- ) }, \\
  S_\B(\xA^+, \xB^+)
  &= \frac{ \exp(\tau_t^2 \fA^+ \cdot \fB^+ ) }
    {\exp(\tau_t^2 \fA^+ \cdot \fB^+ ) + K \E_{\xA^-} \exp(\tau_t^2 \fA^- \cdot \fB^+ ) },
\end{align*}
where $K > 0$ controls the strength of negative samples and $\tau_t \in [0, 1]$ is a non-decreasing 
value representing the inverse temperature. Then, we define the loss as 
\[
  \Loss 
  := \Loss_\A + \Loss_\B 
  := - \E \log S_\A(\xA^+, \xB^+) - \E \log S_\A(\xA^+, \xB^+).
\]



\subsection{Gradients}
Now, we compute the gradient of $\Loss$ w.r.t.~$\WA$ and $\WB$. The proof of this lemma is 
deferred to the end of this subsection. 


\begin{align*}
  \Q_1
  &:= \E \braces{
      \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
      \z^+(\z^+)\trans d
    } \\
    &\qquad
    - K \E \braces{
      \frac{ S_\A(\xA^+, \xB^+) \exp( \fA^+ \cdot \fB^-)}{\exp( \fA^+ \cdot \fB^+)}
      \z^- (\z^+)\trans d
    } 
    - K \E \braces{
      \frac{S_\B(\xA^+, \xB^+) \exp( \fA^- \cdot \fB^+)}{\exp( \fA^+ \cdot \fB^+)}
      \z^+ (\z^-)\trans d
    }
\end{align*}

\begin{lemma}
  \label{lemma: grad Loss}
  We have
  \begin{align*}
    \nabla_{\WA} \Loss
    &= - \tau_t^2 
      \E_{\xA^+, \xB^+} \braces{ 
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \left(
          \frac{\xA^+(\fB^+)\trans}{N_\A}
          - \inprod{\fA^+}{\fB^+} 
            \frac{\left(\A\KA\trans + \A_{\bxi}\KAxi\trans \right)}{ N_\A^2 d }
        \right)
      } \\
      &\qquad
      + \frac{K \tau_t^2 }{N_\A}
      \E_{\xA^+, \xB^\pm} \braces{ 
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \left(
          \xA^+(\fB^-)\trans
          - \inprod{\fA^+}{\fB^-} 
            \frac{\left(\A\KA\trans + \A_{\bxi}\KAxi\trans \right) / \sqrt{d}}
                 { \sqrt{\norm{\KA}_F^2 + \norm{\KAxi}_F^2} }
        \right)
      } \\
      &\qquad
      + \frac{ K \tau_t^2 }{ N_\A }
      \E_{\xA^\pm, \xB^+} \braces{ 
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
          \left(
            \xA^-(\fB^+)\trans
            - \inprod{\fA^-}{\fB^+} 
              \frac{\left(\A\KA\trans + \A_{\bxi}\KAxi\trans \right) / \sqrt{d}}
                   { \sqrt{\norm{\KA}_F^2 + \norm{\KAxi}_F^2} }
          \right)
      }.
  \end{align*}
  The formula for $\nabla_{\WB} \Loss$ can be obtained by interchanging the roles of $\A$ and $\B$.
\end{lemma}



Instead of tracking $\WA$ and $\WB$ directly, we are going to track $\KA$, $\KB$, $\KAxi$ and 
$\KBxi$. The dynamics of them is governed by the following equation. As a direct corollary of 
Lemma~\ref{lemma: grad Loss}, we have the following. 

\begin{lemma}
  \label{lemma: d KA, d KAxi}
  We have
  \begin{align*}
    \frac{\rd}{\rd t} \KA 
    &= \tau_t^2
      \E_{\xA^+, \xB^+} \braces{ 
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \left(
          \frac{ (\KB\z^+ + \KBxi\bxi_\B) (\z^+)\trans }{N_\A N_\B}
          - \inprod{\fA^+}{\fB^+}\frac{\KA}{ N_\A^2 d}
        \right)
      } \diag(\bsigma^2)
      \\
      &\qquad
      - K \tau_t^2
      \E_{\xA^+, \xB^\pm} \braces{ 
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \left(
          \frac{ \fB^-(\z^+)\trans }{N_\A}
          - \inprod{\fA^+}{\fB^-}  \frac{\KA}{ N_\A^2 d }
        \right)
      } \diag(\bsigma^2) \\
      &\qquad
      - K \tau_t^2 
      \E_{\xA^\pm, \xB^+} \braces{ 
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
          \left(
            \frac{ \fB^+(\z^-)\trans }{N_\A}
            - \inprod{\fA^-}{\fB^+} \frac{ \KA }{ N_\A^2 d }
          \right)
      } \diag(\bsigma^2),
  \end{align*}
  and 
  \begin{align*}
    \frac{\rd}{\rd t} \KAxi
    &= \frac{\tau_t^2 }{N_\A}
      \E_{\xA^+, \xB^+} \braces{ 
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \left(
          \fB^+(\bxi_\A^+)\trans 
          - \frac{ \inprod{\fA^+}{\fB^+}  \KAxi / \sqrt{d}}
                 { \sqrt{\norm{\KA}_F^2 + \norm{\KAxi}_F^2} }
        \right)
      } \sigma_\xi^2 \\
      &\qquad
      - \frac{K \tau_t^2 }{N_\A}
      \E_{\xA^+, \xB^\pm} \braces{ 
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \left(
          \fB^-(\bxi_\A^+)\trans
          - \frac{ \inprod{\fA^+}{\fB^-}  \KAxi / \sqrt{d}}
                 { \sqrt{\norm{\KA}_F^2 + \norm{\KAxi}_F^2} }
        \right)
      } \sigma_\xi^2 \\
      &\qquad
      - \frac{ K \tau_t^2 }{ N_\A }
      \E_{\xA^\pm, \xB^+} \braces{ 
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
          \left(
            \fB^+(\bxi_\A^-)\trans
            - \frac{ \inprod{\fA^-}{\fB^+} \KAxi / \sqrt{d}}
                   { \sqrt{\norm{\KA}_F^2 + \norm{\KAxi}_F^2} }
          \right)
      } \sigma_\xi^2.
  \end{align*}
\end{lemma}

We can rewrite the above result as follows. 
\begin{corollary}
  \label{cor: dynamics, Q}
  Define 
  \begin{align*}
    Q_0
    &:= 
      - \E_{\xA^+, \xB^+} \braces{ 
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \inprod{\fA^+}{\fB^+} 
      } \\
      &\qquad
      + K 
      \E_{\xA^+, \xB^\pm} \braces{ 
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \inprod{\fA^+}{\fB^-} 
      } 
      + K 
      \E_{\xA^\pm, \xB^+} \braces{ 
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \inprod{\fA^-}{\fB^+} 
      },
  \end{align*}
  and 
  \begin{align*}
    \Q_1
    &:= \E \braces{
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \z^+(\z^+)\trans d
      } \\
      &\qquad
      - K \E \braces{
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \z^- (\z^+)\trans d
      } 
      - K \E \braces{
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \z^+ (\z^-)\trans d
      }, \\
    \Q_{1, \xi_\B}
    &:= \E \braces{
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \bxi_\B^+(\z^+)\trans d
      } \\
      &\qquad
      - K \E \braces{
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\B^- (\z^+)\trans d
      } 
      - K \E \braces{
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\B^+ (\z^-)\trans d
      }, \\
    \Q_{1, \xi_\A}
    &:= \E \braces{
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \bxi_\A^+(\z^+)\trans d
      } \\
      &\qquad
      - K \E \braces{
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\A^+ (\z^-)\trans d
      } 
      - K \E \braces{
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\A^- (\z^+)\trans d
      }, \\
    \Q_2
    &:= \E \braces{
        \left( 2 - S_\A(\xA^+, \xB^+) - S_\B(\xA^+, \xB^+) \right)
        \bxi_\B^+ (\bxi_\A^+)\trans d
      } \\
      &\qquad
      - K \E \braces{
        \frac{ S_\A(\xA^+, \xB^+) \exp(\tau_t^2 \fA^+ \cdot \fB^-)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\B^- (\bxi_\A^+)\trans d 
      }
      - K \E \braces{ 
        \frac{S_\B(\xA^+, \xB^+) \exp(\tau_t^2 \fA^- \cdot \fB^+)}{\exp(\tau_t^2 \fA^+ \cdot \fB^+)}
        \bxi_\B^+(\bxi_\A^-)\trans d
      }.
  \end{align*}
  We have \TODO{For notational simplicity, we rescale the gradients by $\tau_t^{-2}$. Need to 
  divide all formulas in Stage~1 by $\tau_t^2$.}
  \begin{align*}
    \frac{\rd}{\rd t} \KA 
    &= \frac{\KB}{N_\A N_\B d} \Q_1 \diag(\bsigma^2) 
      + \frac{\KBxi}{N_\A N_\B d} \Q_{1, \xi_\B} \diag(\bsigma^2) 
      + \frac{\KA}{N_\A^2 d} Q_0 \diag(\bsigma^2), \\
    \frac{\rd}{\rd t} \KB 
    &= \frac{\KA}{N_\A N_\B d} \Q_1\trans \diag(\bsigma^2) 
      + \frac{\KAxi}{N_\A N_\B d} \Q_{1, \xi_\A} \diag(\bsigma^2) 
      + \frac{\KB}{N_\B^2 d} Q_0 \diag(\bsigma^2), \\
    \frac{\rd}{\rd t} \KAxi
    &= \frac{ \KB }{ N_\A N_\B d} \Q_{1, \bxi_\A}\trans \sigma_\xi^2
      + \frac{\KBxi}{N_\A N_\B d} \Q_2 \sigma_\xi^2
      + \frac{\KAxi}{N_\A^2 d} Q_0 \sigma_\xi^2, \\
    \frac{\rd}{\rd t} \KBxi
    &= \frac{ \KA }{ N_\A N_\B d } \Q_{1, \bxi_\B}\trans \sigma_\xi^2
      + \frac{ \KAxi }{ N_\A N_\B d } \Q_2\trans \sigma_\xi^2 
      + \frac{\KBxi}{N_\B^2 d} Q_0 \sigma_\xi^2. 
  \end{align*}
\end{corollary}


We are interested in each column of $\KA$ and $\KB$, whose dynamics is given by the next lemma. 
The next lemma also decompose the dynamics along the radial and tangent directions. 
\begin{lemma}
  \label{lemma: d norm and d bar}
  For an $p \in [r]$ and $q \in [d-r]$, we have 
  \begin{align*}
    \frac{\rd}{\rd t} \norm{[\KA]_p}^2
    &= 2 \frac{\inprod{[\KA]_p}{[\KB\Q_1]_p}}{N_\A N_\B d} \sigma_p^2
      + 2 \frac{\inprod{[\KA]_p}{[\KBxi\Q_{1, \xi_\B}]_p}}{N_\A N_\B d}  \sigma_p^2
      + 2 \frac{\norm{[\KA]_p}^2}{N_\A^2 d} Q_0 \sigma_p^2, \\
    \frac{\rd}{\rd t} \norm{[\KB]_p}^2
    &= 2 \frac{ \inprod{[\KB]_p}{[\KA\Q_1\trans]_p}}{N_\A N_\B d} \sigma_p^2
      + 2 \frac{ \inprod{[\KB]_p}{[\KAxi\Q_{1, \xi_\A}]_p}}{N_\A N_\B d}  \sigma_p^2
      + 2 \frac{\norm{[\KB]_p}^2}{N_\B^2 d} Q_0 \sigma_p^2, \\
    \frac{\rd}{\rd t} \norm{[\KAxi]_q}^2
    &= 2 \frac{ \inprod{[\KAxi]_q}{[\KB \Q_{1, \bxi_\A}\trans]_q} }{ N_\A N_\B d}  \sigma_\xi^2
      + 2 \frac{ \inprod{[\KAxi]_q}{[\KBxi \Q_2]_q} }{N_\A N_\B d} \sigma_\xi^2
      + 2 \frac{\norm{[\KAxi]_q}_F^2}{N_\A^2 d} Q_0 \sigma_\xi^2, \\
    \frac{\rd}{\rd t} \norm{[\KBxi]_q}^2
    &= 2 \frac{ \inprod{[\KBxi]_q}{[\KA \Q_{1, \bxi_\B}\trans]_q} }{ N_\A N_\B d } \sigma_\xi^2
      + 2 \frac{ \inprod{[\KBxi]_q}{[\KAxi \Q_2\trans]_q} }{ N_\A N_\B d } \sigma_\xi^2 
      + 2 \frac{\norm{[\KBxi]_q}^2}{N_\A^2 d} Q_0 \sigma_\xi^2,
  \end{align*}
  and 
  \begin{align*}
    \frac{\rd}{\rd t} \ol{ [\KA]_p }
    &= \left( \Id - \ol{ [\KA]_p } \left( \ol{ [\KA]_p } \right)\trans  \right)
      \left(
        \frac{[\KB \Q_1]_p }{ \norm{[\KA]_p} }
        + \frac{[\KBxi \Q_{1, \xi_\B}]_p}{\norm{[\KA]_p} }
      \right)
      \frac{\sigma_p^2 }{N_\A N_\B d }, \\
    \frac{\rd}{\rd t} \ol{ [\KB]_p }
    &= \left( \Id - \ol{ [\KB]_p } \left( \ol{ [\KB]_p } \right)\trans  \right)
      \left(
        \frac{[\KA \Q_1\trans]_p }{ \norm{[\KB]_p} }
        + \frac{[\KAxi \Q_{1, \xi_\A}]_p }{ \norm{[\KB]_p} }
      \right)
      \frac{\sigma_p^2 }{N_\A N_\B d }, \\
    \frac{\rd}{\rd t} \ol{ [\KAxi]_q }
    &= \left( \Id - \ol{ [\KAxi]_q } \left( \ol{ [\KAxi]_q } \right)\trans \right)
      \left(
        \frac{ [\KB \Q_{1, \bxi_\A}\trans]_q }{ \norm{[\KAxi]_q} }
        + \frac{ [\KBxi \Q_2]_q }{ \norm{[\KAxi]_q} }
      \right) 
      \frac{\sigma_\xi^2 }{N_\A N_\B d }, \\
    \frac{\rd}{\rd t} \ol{ [\KBxi]_q }
    &= \left( \Id - \ol{ [\KBxi]_q } \left( \ol{ [\KBxi]_q } \right)\trans \right)
      \left(
        \frac{ [\KA \Q_{1, \bxi_\B}\trans]_q }{ \norm{[\KBxi]_q} }
        + \frac{ [\KAxi \Q_2\trans]_q }{ \norm{[\KBxi]_q} }
      \right) 
      \frac{\sigma_\xi^2 }{N_\A N_\B d }. 
  \end{align*}
\end{lemma}













